Smart Contract Development from the Perspective of Developers: Topics and Issues Discussed on Social Media

Blockchain-based platforms are emerging as a transformative technology that can provide reliability, integrity, and auditability without trusted entities. One of the key features of these platforms is the trustworthy decentralized execution of general-purpose computation in the form of smart contracts, which are envisioned to have a wide range of applications. As a result, a rapidly growing and active community of smart-contract developers has emerged in recent years. A number of research efforts have investigated the technological challenges that these developers face, introducing a variety of tools, languages, and frameworks for smart-contract development, focusing on security. However, relatively little is known about the community itself, about the developers, and about the issues that they face and discuss. To address this gap, we study smart-contract developers and their discussions on two social media sites, Stack Exchange and Medium. We provide insight into the trends and key topics of these discussions, into the developers' interest in various security issues and security tools, and into the developers' technological background.

==> PlotsSE/ProfileAgeReputaionComparison.tex <==
\begin{figure}[ht!]
\pgfplotstableread[col sep = comma]{Data/ProfileAgeComparison.csv}\table

\centering
    \begin{subfigure}[b]{.5\linewidth}

      \centering
        \begin{tikzpicture}
            \begin{axis}[
                SmallBarPlot,
                 width=0.4\textwidth,
                 height=2.5cm,
                xticklabels from table={\table}{Years},
                x tick label style={rotate=90,anchor=east},
                % legend style={font=\fontsize{4}{5}\selectfont},
                ylabel=Fractions of users,
                xlabel=Registration dates
            ]
                \addplot [BlueBars] table [x expr=\coordindex, y=PercentageSC] {\table};
                \addlegendentry{Smart Contracts}
                
                \addplot [RedBars] table [x expr=\coordindex, y=PercentageGU] {\table};
                \addlegendentry{General StackOverflow}
            \end{axis}
        \end{tikzpicture}
    %   \caption{Number of answers}
\end{subfigure}%
\pgfplotstableread[col sep = comma]{Data/ReputationComparison.csv}\table%
\begin{subfigure}[b]{.5\linewidth}
      \centering
        \begin{tikzpicture}
            \begin{axis}[
                SmallBarPlot,
                 width=0.4\textwidth,
                 height=2.5cm,
                xticklabels from table={\table}{Reputation},
                ylabel=Fractions of users on Log scale,
                xlabel=Reputation
            ]
                \addplot [BlueBars] table [x expr=\coordindex, y=PercentageSC] {\table};
                \addlegendentry{Smart Contracts}
                \addplot [RedBars] table [x expr=\coordindex, y=PercentageGU] {\table};
                \addlegendentry{General StackOverflow}
            \end{axis}
        \end{tikzpicture}
    %   \caption{Number of answers}
    \end{subfigure}
  \caption{Profile creation dates and reputation of smart contract developers and other Stack Overflow users.}
\label{fig:SO_ProfileCreation_ReputationComparison}
\end{figure}

==> Tables/MostFrequentTags_Medium.tex <==

% \vspace*{-1pt}
\begin{table}[h]
    \caption{Most Frequent Tags in Smart Contract Related Posts on Medium}
    \label{tab:popularity_matrix}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
\hline
    \multirow{2}{*}{\textbf{Tags}} & \multirow{2}{*}{\textbf{Number}} & \multicolumn{3}{c|}{\textbf{Average}} \\
    \cline{3-5}
     &  & \textbf{Responses} & \textbf{Claps} & \textbf{Voters}  \\ \hline \hline
      Ethereum  &  2643 &  2.37 &  388.03 &  37.1 \\ \hline
      Blockchain & 2585 &  2.06 &  423.2 & 35.91\\ \hline
      Smart Contracts & 1274 & 1.68 &  310.5 &  32.03  \\ \hline
      Solidity & 907 &  1.62 &  290.28 &  29.26 \\ \hline
      Cryptocurrency & 659 & 2.48 &  577.43 &  41.32 \\ \hline
      Security & 476 &  0.81 &  193.59 &  16.5 \\ \hline
      Erc20 & 467 &  3.63 &  836.46 &  54.46 \\ \hline
      Web3 & 401 &  1.75 &  429.34 &  41.03 \\ \hline
      Bitcoin & 369 &  5.04 &  730.14 &  74.07 \\ \hline
      Metamask & 296 &  0.76 &  216.02 &  16.97 \\ \hline
    %   ICO & 265 &  2.4 &  656.12 &  46.12 \\ \hline
    %   Dapps & 250 &  2 &  424 &  36 \\ \hline
    %   Truffle & 185 &  1.13 &  104.64 &  11.9 \\ \hline
    %   Programming & 132 & 1.71 &  414.32 &  42.5 \\ \hline
    %   Audit & 119 &  0.31 &  141.17 &  9.95 \\ \hline
    %   Decentralization & 117 &  1.63 &  496.72 & 37.38 \\ \hline
\end{tabular}
\end{table}

==> Tables/MostFrequentTags_SE.tex <==

\begin{table}
\caption{Most Frequent Tags in Smart Contract Related Questions on Stack Exchange}
\label{tab:SO_Popular_TagFrequency}

     \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    
    \multirow{2}{*}{\textbf{Tags}} & \multirow{2}{*}{\textbf{Number}} & \multicolumn{4}{c|}{\textbf{Average}} \\
    \cline{3-6}
     &  & \textbf{Scores} & \textbf{Views} & \textbf{Answers} & \textbf{Comments} \\ \hline \hline
     
    %  \multirow{2}{*}{\textbf{Tags}} & \multirow{2}{*}{\textbf{Number}}& \multirow{2}{*}{\textbf{Scores}}& \multirow{2}{*}{\textbf{Views}} & \multirow{2}{*}{\textbf{Answers}} & \multirow{2}{*}{\textbf{Comments}} \\ 
    %  & & (avg.)    &   (avg.) &     (avg.) &    (avg.) \\ \hline \hline


Solidity & 9323 & 0.48& 751.92 & 1.2& 1.14 \\
 \hline 
 Go-ethereum & 4946 & 0.55& 1046.71 & 1.09& 1.19 \\
 \hline 
 Web3js & 3948 & 0.48& 879.77 & 1.16& 1.37 \\
 \hline 
 Contract-development & 2973 & 0.7& 844.59 & 1.29& 1.04 \\
 \hline 
 Blockchain & 2539 & 0.88& 1232.09 & 1.53& 1.37 \\
 \hline 
 Ethereum & 2530 & 1.55& 3023.0 & 3.73& 3.94 \\
 \hline 
 Truffle & 2430 & 0.4& 750.02 & 1.28& 1.46 \\
 \hline 
 Transactions & 1743 & 0.94& 1382.02 & 1.31& 1.1 \\
 \hline 
 Remix & 1642 & 0.29& 592.96 & 1.15& 1.34 \\
 \hline 
 Contract-design & 1522 & 1.12& 872.72 & 1.34& 0.92 \\

 \hline 
\end{tabular}
\end{table}
